Increasing Missingness to Reduce Bias: Richardson-SGD with Missing Data

Stochastic gradient methods are central to modern large-scale learning, but their use with incomplete covariates remains delicate since imputation schemes generally introduce systematic gradient biases, as shown for linear models. In this work, we prove that all parametric models exhibit similar gradient bias for various imputation procedures and characterize exactly the dependence on the missingness ratio vector $p$, with $O(\|p\|)$ as the leading term. We exploit this analysis to propose a simple debiasing procedure for stochastic gradient descent (SGD) with missing values based on Richardson extrapolation, which leverages the exact expression of the gradient bias. The key idea is to \emph{deliberately add missingness}: from an already incomplete observation, we generate a further-thinned version at a higher, controlled missingness level, and combine the two resulting stochastic gradients to cancel the leading bias term. We prove that one Richardson step reduces the gradient bias from $O(\|p\|)$ to $O(\|p\|^2)$ under several missingness scenarios. Our proposed method is computationally efficient, model-agnostic and applies to any parametric loss whose stochastic gradient can be computed after imputation. Furthermore, when missing indicators are independent, the population gradient bias is a multilinear polynomial in $p$ and depends only on population gradient errors induced by declaring a single coordinate missing. In this case, our method generalizes to a multi-step Richardson procedure which recursively cancels higher-order terms. Empirically, Richardson debiasing improves optimization and estimation across several generalized linear models and combines positively with widely used imputation procedures such as MICE. These results suggest that, somewhat counter-intuitively, adding controlled missingness on top of existing missing data can make stochastic learning from incomplete data more accurate.

==> checklist.tex <==
%\section*{NeurIPS Paper Checklist}


% \begin{enumerate}

% \item {\bf Claims}
%     \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
%     \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: Proofs and numerical experiments are given to support our claims. 

% \item {\bf Limitations}
%     \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
%     \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: The limitations, such as assumption, or limits of our theory are given in the main text.


% \item {\bf Theory assumptions and proofs}
%     \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
%     \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: Assumptions and proofs are given for all the results. 

% \item {\bf Experimental result reproducibility}
%     \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
%     \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: Details on the experiments are given in the appendix.

% \item {\bf Open access to data and code}
%     \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
%     \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: Details on the experiments are sufficent to reproduce similar results. Moreover, a code repository will be given once the paper is no more under anonymous review.


% \item {\bf Experimental setting/details}
%     \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
%     \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: All parameters, like the number of points or the regularization are stated.

% \item {\bf Experiment statistical significance}
%     \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
%     \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: Experiments are reproduce several time, and the averaged results are displayed, along their standard deviations.
   
% \item {\bf Experiments compute resources}
%     \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
%     \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: Experiments are done on a simple modern CPU, there is no specific resources needed. 
   
% \item {\bf Code of ethics}
%     \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
%     \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification:  The research complies with the NeurIPS Code of Ethics. It is methodological, uses synthetic data only, and does not involve human subjects, personal data, sensitive attributes, or deployed systems.


% \item {\bf Broader impacts}
%     \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
%     \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: The paper is theoretical and methodological, uses only 
% synthetic data. A discussion of broader societal impacts is 
% not applicable.
    
% \item {\bf Safeguards}
%     \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
%     \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: Non applicable.


% \item {\bf Licenses for existing assets}
%     \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
%     \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: All paper and libraries used are cited.

% \item {\bf New assets}
%     \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
%     \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: The paper does not release new assets.

% \item {\bf Crowdsourcing and research with human subjects}
%     \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
%     \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: Non applicable.

% \item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
%     \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
%     \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: Non applicable.

% \item {\bf Declaration of LLM usage}
%     \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
%     %this research? 
%     \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: Non applicable.
    
% \end{enumerate}

==> miscellaneous_results.tex <==

\section{Proof of Proposition \ref{prop:grad_bias_fo_struct} - First-order structure of the missingness bias}
\fg{A réécrire proprement, version complète de la prop dans le corps du texte. }
\textbf{Proposition} \ref{prop:grad_bias_fo_struct}( Exact First-order structure of the missingness bias)
Let $M^{(p)}=(M_1^{(p)},\dots,M_d^{(p)})\in\{0,1\}^d$ be a missingness mask,
where $M_j^{(p)}=1$ means that coordinate $j$ is missing. Let
\[
    g(w;x,y):=\nabla_w\ell(w;x,y)\in\mathbb R^q .
\]
For $S\subseteq[d]$, define $x^{\mathrm{NA},S}$ by setting $x_j=\mathrm{NA}$
for $j\in S$, and define
\[
    G_S(w;x,y,U,\xi)
    :=
    \nabla_w\ell\left(
        w;\mathcal I(x^{\mathrm{NA},S},U,\xi),y
    \right),
\]
where $\mathcal I$ is an arbitrary imputation or preprocessing rule. If
$\mathcal I$ is random, assume
\[
    \xi\perp M^{(p)}\mid (X,Y,U).
\]
Let
\[
    T_jG_S:=G_{S\cup\{j\}},
    \qquad
    \Delta_j:=T_j-I,
    \qquad
    \Delta_S:=\prod_{j\in S}\Delta_j,
    \qquad
    \Delta_\varnothing:=I.
\]

For $S\subseteq[d]$, define the conditional co-missingness moment
\[
    \rho_S^{(p)}(x,y,U)
    :=
    \mathbb E\left[
        \prod_{j\in S}M_j^{(p)}
        \,\middle|\,
        X=x,Y=y,U
    \right],
    \qquad
    \rho_\varnothing^{(p)}(x,y,U):=1.
\]
Equivalently,
\[
    \rho_S^{(p)}(x,y,U)
    =
    \mathbb P(M_j^{(p)}=1 \ \forall j\in S\mid X=x,Y=y,U).
\]

Then, without assuming conditional independence of
$M_1^{(p)},\dots,M_d^{(p)}$, the conditional gradient bias is
\[
    B(p)
    :=
    \mathbb E_M
    \left[
        G_{S(M^{(p)})}(w;x,y,U,\xi)
        \mid x,y,U,\xi
    \right]
    -
    G_\varnothing(w;x,y,U,\xi)
    =
    \sum_{\varnothing\neq S\subseteq[d]}
    \rho_S^{(p)}(x,y,U)\,
    \Delta_SG_\varnothing(w;x,y,U,\xi).
\]
Thus higher-order cross terms are present through the joint co-missingness
coefficients $\rho_S^{(p)}$ for $|S|\ge2$.


\begin{proof}
Fix $x,y,U,\xi$. For a realized mask $m$, write
\[
    S(m):=\{j:m_j=1\}.
\]
Since $T_j$ declares coordinate $j$ missing,
\[
    I+m_j\Delta_j
    =
    \begin{cases}
        I, & m_j=0,\\
        T_j, & m_j=1.
    \end{cases}
\]
Therefore,
\[
    G_{S(m)}
    =
    \left(
        \prod_{j=1}^d (I+m_j\Delta_j)
    \right)G_\varnothing.
\]
Because the operators $\Delta_j$ commute,
\[
    G_{S(m)}
    =
    \sum_{S\subseteq[d]}
    \left(
        \prod_{j\in S}m_j
    \right)
    \Delta_SG_\varnothing.
\]
Taking expectation with respect to $M^{(p)}$, conditionally on $x,y,U,\xi$, gives
\[
\begin{aligned}
    \mathbb E_M
    \left[
        G_{S(M^{(p)})}
        \mid x,y,U,\xi
    \right]
    &=
    \sum_{S\subseteq[d]}
    \mathbb E_M
    \left[
        \prod_{j\in S}M_j^{(p)}
        \,\middle|\,
        x,y,U,\xi
    \right]
    \Delta_SG_\varnothing .
\end{aligned}
\]
Since $\xi\perp M^{(p)}\mid(X,Y,U)$,
\[
    \mathbb E_M
    \left[
        \prod_{j\in S}M_j^{(p)}
        \,\middle|\,
        x,y,U,\xi
    \right]
    =
    \rho_S^{(p)}(x,y,U).
\]
The term $S=\varnothing$ equals $G_\varnothing$. Subtracting it gives
\[
    B(p)
    =
    \sum_{\varnothing\neq S\subseteq[d]}
    \rho_S^{(p)}(x,y,U)\Delta_SG_\varnothing.
\]
No independence among the coordinates of $M^{(p)}$ was used.
\end{proof}

\begin{remark}[Dependent MCAR, sMAR, and sMNAR]
The three mechanisms differ only through the form of
$\rho_S^{(p)}(x,y,U)$.

\medskip

\noindent\textbf{Dependent MCAR.}
If
\[
    M^{(p)}\perp (X,Y,U),
\]
but the coordinates $M_1^{(p)},\dots,M_d^{(p)}$ are not necessarily independent,
then
\[
    \rho_S^{(p)}(x,y,U)
    =
    \rho_S^{(p)}
    :=
    \mathbb P(M_j^{(p)}=1\ \forall j\in S).
\]
Hence
\[
    B_{\mathrm{MCAR}}(p)
    =
    \sum_{\varnothing\neq S\subseteq[d]}
    \rho_S^{(p)}\Delta_SG_\varnothing .
\]
The first terms are
\[
\begin{aligned}
    B_{\mathrm{MCAR}}(p)
    &=
    \sum_{j=1}^d
    \rho_{\{j\}}^{(p)}\Delta_jG_\varnothing
    +
    \sum_{1\le j<k\le d}
    \rho_{\{j,k\}}^{(p)}
    \Delta_{\{j,k\}}G_\varnothing
    \\
    &\quad
    +
    \sum_{1\le j<k<\ell\le d}
    \rho_{\{j,k,\ell\}}^{(p)}
    \Delta_{\{j,k,\ell\}}G_\varnothing
    +\cdots .
\end{aligned}
\]
If the marginal missingness probabilities are $p_j$, then
\[
    \rho_{\{j\}}^{(p)}=p_j,
\]
but, without independence,
\[
    \rho_{\{j,k\}}^{(p)}
    \neq
    p_jp_k
\]
in general.

\medskip

\noindent\textbf{Dependent sMAR.}
Assume
\[
    M^{(p)}\perp (X,Y)\mid U,
\]
and
\[
    \mathbb P(M_j^{(p)}=1\mid U)=p_jq_j(U).
\]
No conditional independence among the coordinates is assumed. Then
\[
    \rho_S^{(p)}(x,y,U)
    =
    \rho_S^{(p)}(U)
    :=
    \mathbb P(M_j^{(p)}=1\ \forall j\in S\mid U),
\]
and
\[
    B_{\mathrm{sMAR}}(p;U)
    =
    \sum_{\varnothing\neq S\subseteq[d]}
    \rho_S^{(p)}(U)\Delta_SG_\varnothing .
\]
The first terms are
\[
\begin{aligned}
    B_{\mathrm{sMAR}}(p;U)
    &=
    \sum_{j=1}^d
    p_jq_j(U)\Delta_jG_\varnothing
    \\
    &\quad
    +
    \sum_{1\le j<k\le d}
    \rho_{\{j,k\}}^{(p)}(U)
    \Delta_{\{j,k\}}G_\varnothing
    \\
    &\quad
    +
    \sum_{1\le j<k<\ell\le d}
    \rho_{\{j,k,\ell\}}^{(p)}(U)
    \Delta_{\{j,k,\ell\}}G_\varnothing
    +\cdots .
\end{aligned}
\]
Here
\[
    \rho_{\{j\}}^{(p)}(U)=p_jq_j(U),
\]
but, without conditional independence,
\[
    \rho_{\{j,k\}}^{(p)}(U)
    \neq
    p_jp_kq_j(U)q_k(U)
\]
in general.

\medskip

\noindent\textbf{Dependent sMNAR.}
Assume
\[
    \mathbb P(M_j^{(p)}=1\mid X=x,Y=y,U)
    =
    p_jq_j(U,x_j),
\]
with no conditional independence among the coordinates. Then
\[
    \rho_S^{(p)}(x,y,U)
    =
    \mathbb P(M_j^{(p)}=1\ \forall j\in S\mid X=x,Y=y,U),
\]
and
\[
    B_{\mathrm{sMNAR}}(p;x,U)
    =
    \sum_{\varnothing\neq S\subseteq[d]}
    \rho_S^{(p)}(x,y,U)\Delta_SG_\varnothing .
\]
The first terms are
\[
\begin{aligned}
    B_{\mathrm{sMNAR}}(p;x,U)
    &=
    \sum_{j=1}^d
    p_jq_j(U,x_j)\Delta_jG_\varnothing
    \\
    &\quad
    +
    \sum_{1\le j<k\le d}
    \rho_{\{j,k\}}^{(p)}(x,y,U)
    \Delta_{\{j,k\}}G_\varnothing
    \\
    &\quad
    +
    \sum_{1\le j<k<\ell\le d}
    \rho_{\{j,k,\ell\}}^{(p)}(x,y,U)
    \Delta_{\{j,k,\ell\}}G_\varnothing
    +\cdots .
\end{aligned}
\]
Here
\[
    \rho_{\{j\}}^{(p)}(x,y,U)=p_jq_j(U,x_j),
\]
but, without conditional independence,
\[
    \rho_{\{j,k\}}^{(p)}(x,y,U)
    \neq
    p_jp_kq_j(U,x_j)q_k(U,x_k)
\]
in general.
\end{remark}

\begin{remark}[When is the dependent-mask bias still multilinear in $p$?]
Without independence, the bias is always linear in the joint co-missingness
parameters $\rho_S^{(p)}$, but it is not necessarily multilinear in the marginal
parameters $p_1,\dots,p_d$. To retain a multilinear form in $p$, one needs an
additional scaling assumption, for example
\[
    \rho_S^{(p)}(x,y,U)
    =
    p_S a_S(x,U)\kappa_S(x,y,U),
    \qquad S\neq\varnothing,
\]
where $\kappa_S$ does not depend on $p$ and $\kappa_{\{j\}}=1$. Then
\[
    B(p)
    =
    \sum_{\varnothing\neq S\subseteq[d]}
    p_S a_S(x,U)\kappa_S(x,y,U)\Delta_SG_\varnothing,
\]
which is again multilinear in $p$. The factors $\kappa_S$ encode the dependence
between missingness indicators. In the independent case, $\kappa_S=1$ for all
$S$.
\end{remark}

\section{Proof of Proposition \ref{prop:estimated_richardson} - Richardson under estimated missigness parameters}

\begin{proof}
The effective conditional missingness intensity after the plug-in thinning is
\[
    \tilde\lambda_j(V)
    :=
    \PP(m_j^R=0\mid V).
\]
Since
\[
    \PP(m_j^{(p)}=1\mid V)=1-\lambda_j(V),
\]
and
\[
    \PP(r_j=1\mid V,m^{(p)})
    =
    \frac{1-C\hat\lambda_j(V)}
         {1-\hat\lambda_j(V)},
\]
we have
\[
\begin{aligned}
    1-\tilde\lambda_j(V)
    &=
    \PP(m_j^R=1\mid V) \\
    &=
    \bigl(1-\lambda_j(V)\bigr)
    \frac{1-C\hat\lambda_j(V)}
         {1-\hat\lambda_j(V)}.
\end{aligned}
\]
Therefore
\[
\begin{aligned}
    \tilde\lambda_j(V)
    &=
    1-
    \bigl(1-\lambda_j(V)\bigr)
    \frac{1-C\hat\lambda_j(V)}
         {1-\hat\lambda_j(V)}  \\
    &=
    C\lambda_j(V)
    +
    (C-1)
    \frac{\hat\lambda_j(V)-\lambda_j(V)}
         {1-\hat\lambda_j(V)}.
\end{aligned}
\]
Define the plug-in discrepancy
\[
    e_j^{(C)}(V)
    :=
    \tilde\lambda_j(V)-C\lambda_j(V)
    =
    (C-1)
    \frac{\hat\lambda_j(V)-\lambda_j(V)}
         {1-\hat\lambda_j(V)}.
\]
Thus
\[
    \tilde\lambda=C\lambda+e^{(C)}.
\]

Using the bias expansion,
\[
\begin{aligned}
    \mathbb E[\hat g^{\mathrm R}_{C,\hat\lambda}(w)]
    -
    \nabla L(w)
    &=
    \frac{
        C\mathcal B_w(p)
        -
        \mathcal B_w(\tilde p)
    }
    {C-1}  \\
    &=
    \frac{
        C\mathcal A_w(p)
        -
        \mathcal A_w(C p+e^{(C)})
    }
    {C-1}  \\
    &\quad
    +
    \frac{
        C\mathcal R_w(p)
        -
        \mathcal R_w(Cp+e^{(C)})
    }
    {C-1}.
\end{aligned}
\]
Since \(\mathcal A_w\) is linear,
\[
    C\mathcal A_w(p)
    -
    \mathcal A_w(Cp+e^{(C)})
    =
    -\mathcal A_w(e^{(C)}).
\]
Hence
\[
    \mathbb E[\hat g^{\mathrm R}_{C,\hat\lambda}(w)]
    -
    \nabla L(w)
    =
    -
    \frac{1}{C-1}\mathcal A_w(e^{(C)})
    +
    O\left(
        \|p\|^2
        +
        \|p\|\|e^{(C)}\|
        +
        \|e^{(C)}\|^2
    \right).
\]

It remains to bound \(e^{(C)}\). By definition,
\[
\begin{aligned}
    |\hat\lambda_j(V)-\lambda_j(V)|
    &=
    |\hat p_j\hat q_j(V)-p_jq_j(V)| \\
    &\leq
    |\hat p_j-p_j|\,|q_j(V)|
    +
    |\hat p_j|\,|\hat q_j(V)-q_j(V)| \\
    &\leq
    Q\delta_p
    +
    (\|p\|_\infty+\delta_p)\delta_q.
\end{aligned}
\]
Since \(\hat\lambda_j(V)\leq \rho<1\),
\[
    |e_j^{(C)}(V)|
    \leq
    \frac{C-1}{1-\rho}
    \left[
        Q\delta_p
        +
        (\|p\|_\infty+\delta_p)\delta_q
    \right].
\]
Thus
\[
    \|e^{(C)}\|
    =
    O\left(
        \delta_p
        +
        \|p\|_\infty\delta_q
        +
        \delta_p\delta_q
    \right).
\]
Since \(q_j\) is uniformly bounded,
\[
    \|\lambda\|=O(\|p\|).
\]
Substituting these bounds gives
\[
    \left\|
        \mathbb E[\hat g^{\mathrm R}_{C,\hat\lambda}(w)]
        -
        \nabla L(w)
    \right\|
    =
    O\left(
        \|p\|^2
        +
        \delta_p
        +
        \|p\|_\infty\delta_q
        +
        \delta_p\delta_q
    \right).
\]
\end{proof}

\textcolor{red}{\textbf{RESULTS TO INCORPORATE}}



\newpage 

\section{General results on the gradient bias}

\fg{Changer $0$ par $\mathrm{NA}$ pour être plus général. L'imputation sera quelconque. }

Let
\[
    g(w;x,y) := \nabla_w \ell(w;x,y) \in \RR^q
\]
denote the complete-data single-sample gradient contribution. Here
$x\in\RR^d$, $y$ is the response, and $w$ is the model parameter.

Let
\[
    \omega=(\omega_1,\dots,\omega_d)\in\{0,1\}^d
\]
be the observation mask, where
\[
    \omega_j = 1 \quad \text{means coordinate }j\text{ is observed},
\]
and
\[
    \omega_j = 0 \quad \text{means coordinate }j\text{ is missing}.
\]
The zero-imputed covariate vector is
\[
    z = \omega\odot x.
\]

It is convenient to define the missingness indicators
\[
    m_j := 1-\omega_j,
\]
so that $m_j=1$ means coordinate $j$ is missing. Define the marginal missingness probabilities
\[
    p_j := \EE[m_j] = \PP(\omega_j=0).
\]

Throughout, we assume MCAR in the following sense:
\[
    m \perp (x,y).
\]
We do \emph{not} assume that $m_1,\dots,m_d$ are mutually independent unless explicitly stated.


\fg{Changer ici avec imputation quelconque. Seul hypothèse: l'imputation est indépendante du mask. }

\textbf{Coordinate-zeroing operators}

For each subset $S\subseteq[d]:=\{1,\dots,d\}$, define $x^{(-S)}\in\R^d$ by
\[
    x^{(-S)}_j =
    \begin{cases}
        0, & j\in S,\\
        x_j, & j\notin S.
    \end{cases}
\]
Thus $x^{(-S)}$ is obtained by zeroing exactly the coordinates in $S$.

Define the coordinate-zeroing operator
\[
    T_S g(w;x,y) := g(w;x^{(-S)},y).
\]
For singletons, write $T_j:=T_{\{j\}}$. The operators $T_j$ commute, since zeroing coordinates in different orders gives the same vector.

Define the discrete-difference operators
\[
    \Delta_j := T_j-I,
\]
and, for $S\subseteq[d]$,
\[
    \Delta_S := \prod_{j\in S}\Delta_j,
    \qquad
    \Delta_\varnothing := I.
\]
For example, for $j\neq k$,
\[
\begin{aligned}
    \Delta_{\{j,k\}}g(w;x,y)
    &= g(w;x^{(-j,-k)},y)
       - g(w;x^{(-j)},y) \\
    &\quad - g(w;x^{(-k)},y)
       + g(w;x,y).
\end{aligned}
\]
This is the interaction effect of jointly zeroing coordinates $j$ and $k$.

\textbf{Exact decomposition under general MCAR}

For a realized missingness vector $m$, we can reformulate the masking operator as
\[
    \prod_{j=1}^d (I+m_j\Delta_j).
\]
Indeed, if $m_j=0$, then coordinate $j$ is observed and the factor is $I$. If $m_j=1$, then coordinate $j$ is missing and the factor is $I+\Delta_j = T_j$.
Therefore,
\[
    g(w;\omega\odot x,y)
    =
    \left(\prod_{j=1}^d (I+m_j\Delta_j)\right)g(w;x,y).
\]
Expanding the product gives the pathwise identity
\[
    g(w;\omega\odot x,y)
    =
    \sum_{S\subseteq[d]}
    \left(\prod_{j\in S} m_j\right)
    \Delta_S g(w;x,y).
\]

Define the joint co-missingness probability
\[
    P_{m}(S)
    :=
    \EE\left[\prod_{j\in S}m_j\right]
    =
    \PP(m_j=1\text{ for all }j\in S)
    =
    \PP(\omega_j=0\text{ for all }j\in S),
\]
with the convention $P_m(\varnothing)=1$. In particular,
\[
    P_m(\{j\}) = p_j.
\]

Since $m\perp(x,y)$, conditioning on $(x,y)$ gives
\[
    \EE_m[g(w;\omega\odot x,y)\mid x,y]
    =
    \sum_{S\subseteq[d]}
    P_m(S)\Delta_S g(w;x,y).
\]
Hence the conditional gradient bias is
\[
    \EE_m[g(w;\omega\odot x,y)\mid x,y]-g(w;x,y)
    =
    \sum_{\varnothing\neq S\subseteq[d]}
    P_m(S)\Delta_S g(w;x,y).
\]

This is the fundamental decomposition. It is exact and does not require independence among the coordinates of the mask.

\textbf{Explicit cross terms:} The first few terms are
\[
\begin{aligned}
    &\EE_m[g(w;\omega\odot x,y)\mid x,y]-g(w;x,y) \\
    &\quad =
    \sum_{j=1}^d p_j\Delta_j g(w;x,y) \\
    &\qquad
    + \sum_{1\le j<k\le d}
    P_m(jk)\Delta_{jk}g(w;x,y) \\
    &\qquad
    + \sum_{1\le j<k<\ell\le d}
    P_m(jk\ell)\Delta_{jk\ell}g(w;x,y) \\
    &\qquad
    + \cdots,
\end{aligned}
\]

\section{Population-level bias}
Let
\[
    L(w):=\EE[\ell(w;x,y)]
\]
be the complete-data population risk, and assume that differentiation and expectation can be interchanged, so that
\[
    \nabla L(w)=\EE[g(w;x,y)].
\]
Define
\[
    \mu_S(w):=\EE_{x,y}[\Delta_S g(w;x,y)].
\]
Taking expectation over $(x,y)$, the population gradient bias induced by zero imputation is
\[
    B(w)
    :=
    \EE[g(w;\omega\odot x,y)]-\nabla L(w)
    =
    \sum_{\varnothing\neq S\subseteq[d]}
    P_m(S)\mu_S(w).
\]
Equivalently,
\[
\begin{aligned}
    B(w)
    &=
    \sum_{j=1}^d p_j\mu_j(w) \\
    &\quad
    + \sum_{1\le j<k\le d}P_m(jk)\mu_{jk}(w) \\
    &\quad
    + \sum_{1\le j<k<\ell\le d}P_m(jk\ell)\mu_{jk\ell}(w)
    + \cdots.
\end{aligned}
\]
Thus the bias is linear in the finite-difference functions, but its coefficients are the joint co-missing probabilities of the mask.

\subsection{General form of the bias}

In general, since all the terms are at least linear in $p$, we can see that the bias is of the form 
\[
    B(w) = O(\|p\|) + o(\|p\|) \ . 
\]
We now characterize some specials cases where the form of the bias is more clear. 

\textbf{Coordinatewise independent missingness}

Assume now that $m_1,\dots,m_d$ are mutually independent, with $m_j\sim\B(p_j)$.
Then, for every $S\subseteq[d]$,
\[
    P_m(S)
    =
    \EE\left[\prod_{j\in S}m_j\right]
    =
    \prod_{j\in S}p_j.
\]
Therefore,
\[
    B(w)
    =
    \sum_{\varnothing\neq S\subseteq[d]}
    \left(\prod_{j\in S}p_j\right)\mu_S(w).
\]
The first terms are
\[
\begin{aligned}
    B(w)
    &=
    \sum_{j=1}^d p_j\mu_j(w) \\
    &\quad
    +\sum_{j<k}p_jp_k\mu_{jk}(w) \\
    &\quad
    +\sum_{j<k<\ell}p_jp_kp_\ell\mu_{jk\ell}(w)
    +\cdots.
\end{aligned}
\]
Thus, for fixed $d$ and bounded finite differences,
\[
    B(w)
    =
    \sum_{j=1}^d p_j\mu_j(w)
    +O(\|p\|^2).
\]
In the independent case, the degree of the term $\Delta_S g$ matches $|S|$. Pairwise interactions are quadratic, triple interactions are cubic, and so on.


\textbf{Perfectly correlated missingness indicators}

Consider two coordinates $j$ and $k$ with equal marginal missingness probability $p$, and suppose
\[
    m_j=m_k\sim\B(p).
\]
Then
\[
    P_m(j)=p,
    \qquad
    P_m(k)=p,
\]
but also
\[
    P_m(jk)
    =\EE[m_jm_k]
    =\EE[m_j]
    =p.
\]
The conditional bias terms involving $j,k$ are therefore
\[
    p\Delta_j g(w;x,y)
    +p\Delta_k g(w;x,y)
    +p\Delta_{jk}g(w;x,y).
\]
The pairwise interaction term is not quadratic. It is linear in $p$.

At the population level, the corresponding contribution is
\[
    p\mu_j(w)+p\mu_k(w)+p\mu_{jk}(w).
\]
Thus perfect correlation moves the interaction $\mu_{jk}(w)$ into the first-order bias.


More generally, let $C\subseteq[d]$ be a block of coordinates whose missingness indicators are perfectly correlated:
\[
    m_j = h
    \qquad\text{for all }j\in C,
\]
where
\[
    h\sim\B(p).
\]
Then, for every nonempty subset $S\subseteq C$,
\[
    P_m(S)
    =
    \EE\left[\prod_{j\in S}m_j\right]
    =
    \EE[h^{|S|}]
    =
    \EE[h]
    =p.
\]
Therefore all interaction terms within the block are first order:
\[
    \sum_{\varnothing\neq S\subseteq C}p\mu_S(w)
    =
    p\sum_{\varnothing\neq S\subseteq C}\mu_S(w).
\]
This includes singleton effects, pairwise interactions, triple interactions, and higher-order interactions. None of these terms is suppressed by additional powers of $p$.

Equivalently, if the whole block disappears together with probability $p$, then the first-order bias is the effect of zeroing the whole block:
\[
    p\left(T_C-I\right)g(w;x,y).
\]
Since
\[
    T_C-I
    =
    \prod_{j\in C}(I+\Delta_j)-I
    =
    \sum_{\varnothing\neq S\subseteq C}\Delta_S,
\]
we recover the same expression.






\textcolor{orange}{Remarks: (i)  In general, if we have perfect correlation, or something close to perfect correlation in Bernouilli for the missing vals, it would imply that the whole column is missing or nearly missing and we then discard it. (ii) The bias, from Perfectly correlated missingness for two column, is linear in the missingess probability. }










\section{Linear regression with MCAR missing covariates}

\subsection{Setup and notation}
\fg{Commentaire: commandes fg et erwan}

We work at the \emph{single-observation} level. Thus $x \in \RR^d$ denotes one covariate vector (one row of the dataset), $y \in \RR$ its associated response, and $w \in \RR^d$ the regression parameter.

For squared loss,
\[
\ell(w;x,y)=\frac12 (w^\top x-y)^2,
\]
the gradient contributed by a single observation is
\[
g(w;x,y):=\nabla_w \ell(w;x,y)=(w^\top x-y)x.
\]

For the \emph{population risk},
\[
L(w):=\EE[\ell(w;x,y)],
\]
where $(x,y)$ is drawn from the data-generating distribution. Writing
\[
S:=\EE[xx^\top],
\qquad
b:=\EE[yx],
\]
its gradient is
\[
\nabla L(w)=\EE[g(w;x,y)]=Sw-b.
\]
Hence, if $(x,y)$ is sampled from the population distribution, the single-observation gradient $g(w;x,y)$ is an unbiased estimator of the population gradient $\nabla L(w)$.

Now let $\{(x_i,y_i)\}_{i=1}^n$ be a dataset. The \emph{empirical risk} is
\[
L_n(w):=\frac1n\sum_{i=1}^n \ell(w;x_i,y_i).
\]
Its gradient is
\[
\nabla L_n(w)=\frac1n\sum_{i=1}^n g(w;x_i,y_i).
\]
Therefore, if one index $i$ is drawn uniformly from $\{1,\dots,n\}$, then
\[
\EE_i[g(w;x_i,y_i)] = \nabla L_n(w),
\]
so the gradient from a uniformly sampled observation is also an unbiased estimator of the empirical-risk gradient. 

In what follows, we will not distinguish between the empirical risk and the population risk, and simply refer to the loss as $L$. 



\paragraph{Heterogeneous MCAR missingness.}
For each coordinate $j\in\{1,\dots,d\}$, let
\[
\omega_j \sim \mathrm{Bernoulli}(1-p_j),
\]
where $p_j\in[0,1)$ is the missingness probability of feature $j$. We assume:
\begin{itemize}
    \item $\omega_1,\dots,\omega_d$ are mutually independent,
    \item the mask $m=(\omega_1,\dots,\omega_d)$ is independent of $(x,y)$.
\end{itemize}
The observed covariate vector after \textbf{zero imputation} is
\[
z = m \odot x,
\qquad\text{so that}\qquad
z_j = \omega_j x_j.
\]
The gradient used by SGD, under zero imputation, is therefore
\[
\hat g(w;z,y)=(w^\top z-y)z.
\]

\subsection{Population bias of the zero-imputed gradient}
\paragraph{Sample-conditional bias for a fixed observation.}

We first fix one observation $(x,y)$. All expectations in this subsection are taken only over the mask $m$.

\begin{proposition}[Sample-conditional bias under heterogeneous MCAR]
\label{prop:sample-bias}
Fix $(x,y)\in\RR^d\times\RR$. For each coordinate $j$,
\[
\EE_m[\hat g_j(w;z,y)\mid x,y]-g_j(w;x,y)
=
-p_j x_j^2 w_j
-\sum_{k\neq j}(p_j+p_k-p_jp_k)\,x_jx_k w_k
+p_j yx_j.
\]
Equivalently,
\[
\EE_m[\hat g_j(w;z,y)\mid x,y]-g_j(w;x,y)
=
-p_jg_j(w;x,y)
-(1-p_j)\sum_{k\neq j} p_k\,x_jx_k w_k.
\]
\end{proposition}
\begin{proof}
Recall that $z=\omega\odot x$, so $z_j=\omega_jx_j$. Hence
\[
\hat g_j(w;z,y)
=
\bigl(w^\top z-y\bigr)z_j
=
\Bigl(\sum_{k=1}^d w_k z_k-y\Bigr)z_j
=
\sum_{k=1}^d w_k \omega_j\omega_k x_jx_k - y\omega_jx_j.
\]
Conditioning on $(x,y)$ and taking expectation over $m$ only,
\[
\EE_m[\hat g_j(w;z,y)\mid x,y]
=
\sum_{k=1}^d w_k\,\EE[\omega_j\omega_k]\,x_jx_k
-\EE[\omega_j]\,yx_j.
\]
Under heterogeneous MCAR, the mask coordinates are independent and satisfy
\[
\EE[\omega_j]=1-p_j,
\qquad
\EE[\omega_j\omega_k]=
\begin{cases}
1-p_j, & k=j,\\[1mm]
(1-p_j)(1-p_k), & k\neq j.
\end{cases}
\]
Therefore,
\[
\EE_m[\hat g_j(w;z,y)\mid x,y]
=
(1-p_j)x_j^2w_j
+
\sum_{k\neq j}(1-p_j)(1-p_k)x_jx_kw_k
-(1-p_j)yx_j.
\]
On the other hand,
\[
g_j(w;x,y)=\bigl(w^\top x-y\bigr)x_j
=
x_j(w^\top x)-yx_j
=
x_j^2w_j+\sum_{k\neq j}x_jx_kw_k-yx_j.
\]
Subtracting gives
\[
\EE_m[\hat g_j(w;z,y)\mid x,y]-g_j(w;x,y)
=
-p_j x_j^2 w_j
-\sum_{k\neq j}(p_j+p_k-p_jp_k)x_jx_k w_k
+p_j yx_j,
\]
which is the first formula.

To derive the equivalent form, first rewrite the terms involving $w$:
\[
-p_j x_j^2 w_j
-\sum_{k\neq j}(p_j+p_k-p_jp_k)x_jx_k w_k
=
-p_j\Bigl(x_j^2 w_j+\sum_{k\neq j}x_jx_k w_k\Bigr)
-(1-p_j)\sum_{k\neq j}p_k\,x_jx_k w_k.
\]
Since
\[
x_j^2 w_j+\sum_{k\neq j}x_jx_k w_k = x_j(w^\top x),
\]
this becomes
\[
-p_j x_j^2 w_j
-\sum_{k\neq j}(p_j+p_k-p_jp_k)x_jx_k w_k
=
-p_j x_j(w^\top x)
-(1-p_j)\sum_{k\neq j}p_k\,x_jx_k w_k.
\]
Substituting this into the bias expression yields
\[
\EE_m[\hat g_j(w;z,y)\mid x,y]-g_j(w;x,y)
=
-p_j x_j(w^\top x)
-(1-p_j)\sum_{k\neq j}p_k\,x_jx_k w_k
+p_j yx_j.
\]
Combining the first and last terms, and recalling that $g_j(w;x,y) =\bigl(w^\top x-y\bigr)x_j $, gives the equivalent form.  
\end{proof}

\begin{corollary}[First-order expansion]
\label{cor:first-order}
Fix $(x,y)$. For each $j$,
\[
\EE_m[\hat g_j(w;z,y)\mid x,y]-g_j(w;x,y)
=
-p_j g_j(w;x,y)-\sum_{k\neq j} p_k\,x_jx_k w_k + O(\|p\|^2),
\]
as $\|p\|\to 0$.
\end{corollary}

\begin{proof}
By Proposition~\ref{prop:sample-bias},
\[
\EE_m[\hat g_j(w;z,y)\mid x,y]-g_j(w;x,y)
=
-p_j g_j(w;x,y)
-(1-p_j)\sum_{k\neq j} p_k\,x_jx_k w_k.
\]

Therefore
\[
\EE_m[\hat g_j(w;z,y)\mid x,y]-g_j(w;x,y)
=
-p_j g_j(w;x,y)
-\sum_{k\neq j} p_k\,x_jx_k w_k
+R_j(p),
\]
where
\[
R_j(p):=
p_j\sum_{k\neq j} p_k\,x_jx_k w_k.
\]
It remains to show that $R_j(p)=O(\|p\|^2)$ as $\|p\|\to 0$. Since
\[
R_j(p)=p_j\sum_{k\neq j}p_k\,x_jx_k w_k,
\]
we have
\[
|R_j(p)|
\le
|p_j|\sum_{k\neq j}|p_k|\,|x_jx_k w_k|
\le
\|p\|_\infty^2
\underbrace{\left(|x_j|\sum_{k\neq j}|x_k w_k|\right)}_{=:C_j}.
\]
Thus
\[
|R_j(p)|\le C_j\|p\|_\infty^2,
\]
which concludes the proof by equivalence of norms in $\RR^d$. 
\end{proof}


\paragraph{Population bias of the zero-imputed gradient.}

The population bias is obtained by averaging the sample-conditional bias over the data distribution.

\begin{corollary}[Population bias under heterogeneous MCAR]
\label{cor:population-bias}
Let
\[
B(w):=\EE[\hat g(w;z,y)]-\EE[g(w;x,y)].
\]
For each coordinate $j$,
\[
m_j(w)
=
-p_j\,\nabla_j L(w)
-(1-p_j)\sum_{k\neq j} p_k\,S_{jk}w_k.
\]
In particular, $B(w)=O(\|p\|)$ as $\|p\|\to 0$.
\end{corollary}

\begin{proof}
Taking expectation with respect to the data distribution in Proposition~\ref{prop:sample-bias}, for each coordinate $j$,
\[
m_j(w)
=
\EE\left[\EE_m[\hat g_j(w;z,y)\mid x,y]-g_j(w;x,y)\right].
\]
Using the second form of Proposition~\ref{prop:sample-bias},
\[
\EE_m[\hat g_j(w;z,y)\mid x,y]-g_j(w;x,y)
=
-p_jg_j(w;x,y)
-(1-p_j)\sum_{k\neq j} p_k\,x_jx_k w_k,
\]
we obtain
\[
m_j(w)
=
-p_j\,\EE[g_j(w;x,y)]
-(1-p_j)\sum_{k\neq j} p_k\,\EE[x_jx_k]\,w_k.
\]
Since
\[
\EE[g_j(w;x,y)] = \nabla_j L(w),
\qquad
\EE[x_jx_k]=S_{jk},
\]
it follows that
\[
m_j(w)
=
-p_j\,\nabla_j L(w)
-(1-p_j)\sum_{k\neq j} p_k\,S_{jk}w_k.
\]

We now show that $B(w)=O(\|p\|)$ as $\|p\|\to 0$. For each $j$,
\[
|m_j(w)|
\le
|p_j|\,|\nabla_jL(w)|
+\sum_{k\neq j}|p_k|\,|S_{jk}w_k|
\le
\|p\|_\infty
\left(
|\nabla_jL(w)|+\sum_{k\neq j}|S_{jk}w_k|
\right).
\]
Hence there exists a constant $C(w,S,b)$ such that
\[
\|B(w)\|_\infty \le C(w,S,b)\,\|p\|_\infty.
\]
By equivalence of norms in finite dimension, this implies
\[
\|B(w)\| = O(\|p\|),
\qquad \|p\|\to 0.
\]
\end{proof}


\newpage 

\section{Richardson extrapolation and debiasing }

\textcolor{red}{Now to change, to speak of the general case, and also directly with the coefficients $(p, Cp)$. }

The previous section shows that zero imputation introduces a bias that is first order in the missingness probabilities. We introduce here a \emph{Richardson extrapolation} method to remove the leading order bias.

The basic idea of Richardson extrapolation is as follows. Suppose an estimator $T(p)$, depending on a small parameter $p$, admits an expansion of the form
\[
T(p)=T_0+p\,T_1+p^2\,T_2+O(p^3).
\]
Then the linear combination
\[
T^{\mathrm R}(p):=2T(p)-T(2p)
\]
satisfies
\[
T^{\mathrm R}(p)=T_0-2p^2T_2+O(p^3),
\]
so that the first-order term is eliminated.

More generally, the same idea applies when
\[
T(p)=T_0+p^{\alpha}T_1+p^{\beta}T_2+o(p^{\beta}),
\qquad 0<\alpha<\beta,
\]
in which case one can choose a different linear combination to cancel the leading error term. Likewise, the construction is not restricted to the pair $(p,2p)$: it can be extended to $(p,Cp)$ for any constant $C>0$, with the coefficients adjusted accordingly.


In our setting, $p$ represents the missingness level, and $T(p)$ will be the zero-imputed stochastic gradient under the missingness level $p$. We will construct a Richardson extrapolation scheme, by artificially adding some missing values. 

\subsection{Constructing the extrapolated mask}

Suppose that the data are observed under heterogeneous MCAR with mask
\[
m^{(p)}=(m^{(p)}_1,\dots,m^{(p)}_d),
\qquad
m^{(p)}_j\sim \mathrm{Bernoulli}(1-p_j),
\]
independent across coordinates and independent of $(x,y)$. The corresponding zero-imputed covariate is
\[
z^{(p)}:=m^{(p)}\odot x.
\]

To construct a sample with missingness level $2p=(2p_1,\dots,2p_d)$, we introduce an auxiliary mask, 
\[
r=(r_1,\dots,r_d),
\]
where $r_1, \dots , r_d$ are mutually independent, independent of $(x,y,m^{(p)}$), with
\[
r_j \sim \mathrm{Bernoulli}\left(\frac{1-2p_j}{1-p_j}\right),
\qquad j=1,\dots,d,
\]
which is well-defined provided $p_j<1/2$. \erwan{la condition est un peu bizarre ici. Est-ce que cela ne vaut pas le coup d'écrire le résultat directement dans le cas général avec $Cp$ plutôt que $2p$?}
\fg{Oui je suis d'accord. }We then define the \emph{further-thinned} mask
\[
m^{(2p)}:=m^{(p)}\odot r,
\]
and the associated covariate
\[
z^{(2p)}:=m^{(2p)}\odot x.
\]
Since $m^{(p)}$ and $r$ are independent,
\[
\PP(\omega_j^{(2p)}=1)
=
\PP(\omega_j^{(p)}=1)\PP(r_j=1)
=
(1-p_j)\frac{1-2p_j}{1-p_j}
=
1-2p_j,
\]
so $m^{(2p)}$ is indeed an MCAR mask with missingness probabilities $2p_j$.

We write
\[
\hat g^{(p)}(w):=(w^\top z^{(p)}-y)z^{(p)},
\qquad
\hat g^{(2p)}(w):=(w^\top z^{(2p)}-y)z^{(2p)}.
\]
The Richardson-corrected gradient is then defined by
\[
\hat g^{\mathrm R}(w):=2\hat g^{(p)}(w)-\hat g^{(2p)}(w).
\]


\subsection{Homogeneous MCAR: population-level Richardson cancellation}

Motivated by its simplicity, we will first show the Richardson first order bias cancellation in the homogeneous MCAR setting. That is, we suppose that our missingness vector satisfies
\[
p_1=\cdots=p_d=p,
\qquad p<1/2.
\]
Then the population bias from Corollary~\ref{cor:population-bias} becomes
\[
m_j(w;p)
:=
\EE[\hat g_j^{(p)}(w)]-\nabla_j L(w)
=
-p\,\nabla_j L(w)
-(1-p)p\sum_{k\neq j}S_{jk}w_k.
\]
Equivalently,
\[
m_j(w;p)
=
p\,A_j(w)+p^2\,C_j(w),
\]
where
\[
A_j(w):=-\nabla_jL(w)-\sum_{k\neq j}S_{jk}w_k,
\qquad
C_j(w):=\sum_{k\neq j}S_{jk}w_k.
\]
Thus the population bias is exactly of the form linear term $+$ quadratic term in the scalar parameter $p$, so Richardson extrapolation cancels the entire first-order contribution.

\begin{proposition}[Population Richardson cancellation under homogeneous MCAR]
\label{prop:richardson-homogeneous-pop}
Assume $p_1=\cdots=p_d=p<1/2$, and define
\[
\hat g^{\mathrm R}(w):=2\hat g^{(p)}(w)-\hat g^{(2p)}(w).
\]
Then, for each coordinate $j$,
\[
\EE_m[\hat g_j^{\mathrm R}(w)]-\nabla_jL(w)
=
-2p^2\sum_{k\neq j}S_{jk}w_k = -2p^2C_j(w)
\]
In particular,
\[
\EE_m[\hat g^{\mathrm R}(w)]-\nabla L(w)=O(p^2)
\qquad\text{as }p\to 0.
\]
\end{proposition}

\begin{proof}
Let
\[
m_j(w;p):=\EE[\hat g_j^{(p)}(w)]-\nabla_jL(w).
\]
As noted above,
\[
m_j(w;p)=pA_j(w)+p^2C_j(w),
\]
so
\[
m_j(w;2p)=2pA_j(w)+4p^2C_j(w).
\]
Now, conditioning on $(x,y,m^{(p)})$, and then taking total expectation, we have
\[
\EE[\hat g_j^{\mathrm R}(w)]-\nabla_jL(w)
=
2m_j(w;p)-m_j(w;2p).
\]
Therefore
\[
\EE[\hat g_j^{\mathrm R}(w)]-\nabla_jL(w)
=
2(pA_j+p^2C_j)-(2pA_j+4p^2C_j)
=
-2p^2C_j(w).
\]
\end{proof}

\textbf{When is Richardson extrapolation better: the homogeneous case}
For a fixed coordinate $j$, write
\[
m_j(w;p)=pA_j(w)+p^2C_j(w),
\qquad
B^{\mathrm R}_j(w;p)=-2p^2C_j(w).
\]
We ask when the Richardson-corrected bias is smaller in absolute value than the original zero-imputation bias, that is, when
\[
|B^{\mathrm R}_j(w;p)|<|m_j(w;p)|.
\]
Since $p>0$, this is equivalent to
\[
2p|C_j(w)|<|A_j(w)+pC_j(w)|.
\]
This gives an exact characterization.
\begin{proposition}[When Richardson is better in the homogeneous case]
\label{prop:when-richardson-better-homogeneous}
Fix $w\in\RR^d$ and $j\in\{1,\dots,d\}$. Assume homogeneous MCAR with missingness level $p\in(0,1/2)$. Then:
\begin{itemize}
    \item If $C_j(w)=0$, then $m_j^{\mathrm R}(w;p)=0$, so Richardson extrapolation is always at least as good as the original estimator, and is strictly better whenever $A_j(w)\neq 0$.
    \item If $C_j(w)\neq 0$, then Richardson extrapolation is strictly better on coordinate $j$ if and only if
    \[
    \left|\frac{A_j(w)}{C_j(w)}+p\right|>2p.
    \]
    Equivalently,
    \[
    \frac{A_j(w)}{C_j(w)}>p
    \qquad\text{or}\qquad
    \frac{A_j(w)}{C_j(w)}<-3p.
    \]
\end{itemize}
\end{proposition}
\begin{proof}
By the explicit bias formulas,
\[
|m_j^{\mathrm R}(w;p)|<|m_j(w;p)|
\quad\Longleftrightarrow\quad
2p^2|C_j(w)|<|pA_j(w)+p^2C_j(w)|.
\]
Since $p>0$, dividing by $p$ yields
\[
2p|C_j(w)|<|A_j(w)+pC_j(w)|.
\]
If $C_j(w)=0$, then $m_j^{\mathrm R}(w;p)=0$, and the claim is immediate.
Assume now that $C_j(w)\neq 0$. Dividing by $|C_j(w)|$ gives
\[
2p<\left|\frac{A_j(w)}{C_j(w)}+p\right|.
\]
Finally, for any real number $r$,
\[
|r+p|>2p
\quad\Longleftrightarrow\quad
r>p \ \text{ or } \ r<-3p.
\]
Applying this with $r=A_j(w)/C_j(w)$ concludes the proof.
\end{proof}
\textbf{At the optimum:} useful special case is the optimum $w^\star$, where $\nabla L(w^\star)=0$. Then
\[
A_j(w^\star)=-C_j(w^\star),
\]
hence
\[
m_j(w^\star;p)=pA_j(w^\star)+p^2C_j(w^\star)
=
p(1-p)A_j(w^\star),
\]
while
\[
m_j^{\mathrm R}(w^\star;p)=-2p^2C_j(w^\star)=2p^2A_j(w^\star).
\]
Therefore,
\[
|m_j^{\mathrm R}(w^\star;p)|<|m_j(w^\star;p)|
\quad\Longleftrightarrow\quad
2p^2<p(1-p)
\quad\Longleftrightarrow\quad
p<\frac13.
\]
So, at the optimum, Richardson extrapolation is strictly better whenever the missingness level satisfies $p<1/3$.


\subsection{Heterogeneous MCAR: population-level Richardson cancellation}

We now return to the general heterogeneous case
\[
p=(p_1,\dots,p_d),
\qquad p_j<1/2 \text{ for all }j.
\]
From Corollary~\ref{cor:population-bias}, the population bias of the zero-imputed gradient is
\[
m_j(w;p)
:=
\EE[\hat g_j^{(p)}(w)]-\nabla_jL(w)
=
-p_j\nabla_jL(w)
-(1-p_j)\sum_{k\neq j}p_k\,S_{jk}w_k.
\]
This already exhibits the required linear-plus-quadratic structure:
\[
m_j(w;p)
=
\underbrace{
-p_j\nabla_jL(w)-\sum_{k\neq j}p_k\,S_{jk}w_k
}_{=:L_j(w;p)}
+
\underbrace{
p_j\sum_{k\neq j}p_k\,S_{jk}w_k
}_{=:Q_j(w;p)}.
\]
Here $L_j(w;p)$ is linear in $p$, while $Q_j(w;p)$ is quadratic in $p$.

\begin{proposition}[Population Richardson cancellation under heterogeneous MCAR]
\label{prop:heterogeneous-richardson}
Assume $p_j<1/2$ for all $j$, and define
\[
\hat g^{\mathrm R}(w):=2\hat g^{(p)}(w)-\hat g^{(2p)}(w),
\]
where $\hat g^{(2p)}$ is constructed by the additional thinning scheme above. Then, for each coordinate $j$,
\[
\EE[\hat g_j^{\mathrm R}(w)]-\nabla_jL(w)
=
-2p_j\sum_{k\neq j}p_k\,S_{jk}w_k.
\]
In particular,
\[
\EE[\hat g_j^{\mathrm R}(w)]-\nabla_jL(w)=O(\|p\|^2)
\qquad\text{as }\|p\|\to 0,
\]
whereas the original zero-imputation bias is only $O(\|p\|)$.
\end{proposition}

\begin{proof}
For each coordinate $j$,
\[
m_j(w;p)=L_j(w;p)+Q_j(w;p),
\]
with $L_j$ linear in $p$ and $Q_j$ quadratic in $p$. Hence
\[
L_j(w;2p)=2L_j(w;p),
\qquad
Q_j(w;2p)=4Q_j(w;p).
\]
Moreover,
\[
\EE[\hat g_j^{\mathrm R}(w)]-\nabla_jL(w)
=
2m_j(w;p)-m_j(w;2p).
\]
Therefore
\[
\EE[\hat g_j^{\mathrm R}(w)]-\nabla_jL(w)
=
2(L_j+Q_j)-(2L_j+4Q_j)
=
-2Q_j(w;p).
\]
Substituting the expression for $Q_j$ yields
\[
\EE[\hat g_j^{\mathrm R}(w)]-\nabla_jL(w)
=
-2p_j\sum_{k\neq j}p_k\,S_{jk}w_k.
\]

Finally,
\[
\left|
\EE[\hat g_j^{\mathrm R}(w)]-\nabla_jL(w)
\right|
\le
2\|p\|_\infty^2\sum_{k\neq j}|S_{jk}w_k|,
\]
so the residual bias is $O(\|p\|^2)$ by equivalence of norms in finite dimension.
\end{proof}

\textbf{When we have one or more column where $p_j = 0$:}
Suppose we have $p_j = 0$, in this case $m_j(w,p) = \sum_{k \neq j} p_k S_{jk}w_k$ and thus Richardson debiasing total removes the bias in this coordinate.




\section{Plug-in Richardson correction when the missingness probabilities are estimated}

So far, the Richardson construction assumed that the missingness probabilities
\[
p=(p_1,\dots,p_d)
\]
were known. We study here the case where $p$ is unknown and we replace it by an estimate
\[
\hat p=(\hat p_1,\dots,\hat p_d).
\]
We now study how this affects the population bias of the Richardson-corrected gradient.

When $p$ is unknown, our Richardson scheme uses the estimate $\hat p$ for the auxiliary mask $r = (r_1, \dots, r_d)$, independent of $(x,y,m^{(p)})$, and we have 
\[
r_j\sim \mathrm{Bernoulli}\left(\frac{1-2\hat p_j}{1-\hat p_j}\right),
\qquad j=1,\dots,d.
\]
This is well-defined as long as $\hat p_j<1/2$ for every $j$. The further-thinned mask is then
\[
m^{R} := m^{(p)}\odot r,
\]
and the corresponding covariate is
\[
z^{R} := m^{R}\odot x.
\]

The key point is that this second sample no longer has missingness exactly equal to $2p$. Its effective missingness level is some vector
\[
\tilde p=(\tilde p_1,\dots,\tilde p_d),
\]
which we now compute coordinate by coordinate.

For a fixed coordinate $j$, the first-stage survival probability is $1-p_j$, and the second-stage survival probability is
\[
\frac{1-2\hat p_j}{1-\hat p_j}.
\]
Therefore the overall survival probability after both stages is
\[
\PP(\omega_j^{R}=1)
=
(1-p_j)\frac{1-2\hat p_j}{1-\hat p_j} = 1 - \tilde p_j.
\]
Hence
\[
1-\tilde p_j
=
(1-p_j)\frac{1-2\hat p_j}{1-\hat p_j},
\]
so
\[
\tilde p_j
=
1-(1-p_j)\frac{1-2\hat p_j}{1-\hat p_j}
=
2p_j+\frac{\hat p_j-p_j}{1-\hat p_j}.
\]
It is therefore natural to define the coordinatewise discrepancy
\[
e_j:=\tilde p_j-2p_j=\frac{\hat p_j-p_j}{1-\hat p_j}.
\]
Thus the error made by using $\hat p_j$ instead of $p_j$ in the thinning step shows up as an additive perturbation of the target value $2p_j$.

We now study the resulting Richardson-corrected gradient
\[
\hat g^{\mathrm R}_{\hat p}(w)
:=
2\hat g^{(p)}(w)-\hat g^{R}(w),
\]
where
\[
\hat g^{(p)}(w)=(w^\top z^{(p)}-y)z^{(p)},
\qquad
\hat g^{R}(w)=(w^\top z^{R}-y)z^{R}.
\]

From the earlier population-bias formula, recalling that $S_{jk}:=\EE[x_jx_k]$, for any missingness vector $q=(q_1,\dots,q_d)$ the bias on coordinate $j$ is
\begin{align*}
m_j(w;q)
:&=
\EE[\hat g^{(q)}_j(w)]-\nabla_j L(w) \\
&=
-q_j\,\nabla_j L(w)
-(1-q_j)\sum_{k\neq j} q_k\,S_{jk}w_k \\
&=
-q_j\,\nabla_j L(w)
-\sum_{k\neq j} q_k\,S_{jk}w_k
+
q_j\sum_{k\neq j} q_k\,S_{jk}w_k.
\end{align*}
This separates the bias into a part that is linear in $q$ and a part that is quadratic in $q$.

Applying this first with $q=p$ and then with $q=\tilde p=2p+e$, we get
\[
\EE[\hat g^{\mathrm R}_{\hat p,j}(w)]-\nabla_j L(w)
=
2m_j(w;p)-m_j(w;\tilde p).
\]
We now expand this expression. 
\[
2m_j(w;p)
=
-2p_j\nabla_jL(w)
-2\sum_{k\neq j} p_k S_{jk}w_k
+
2p_j\sum_{k\neq j} p_k S_{jk}w_k.
\]
Since $\tilde p_j=2p_j+e_j$ and $\tilde p_k=2p_k+e_k$,
\[
m_j(w;\tilde p)
=
-(2p_j+e_j)\nabla_jL(w)
-\sum_{k\neq j}(2p_k+e_k)S_{jk}w_k
+
(2p_j+e_j)\sum_{k\neq j}(2p_k+e_k)S_{jk}w_k.
\]

Subtracting gives
\begin{align*}
\EE[\hat g^{\mathrm R}_{\hat p,j}(w)]-\nabla_j L(w)
&=
2m_j(w;p)-m_j(w;\tilde p)\\
&=
e_j\,\nabla_jL(w)
+
\sum_{k\neq j} e_k\,S_{jk}w_k\\
&\quad
-2p_j\sum_{k\neq j} p_k\,S_{jk}w_k
-2p_j\sum_{k\neq j} e_k\,S_{jk}w_k\\
&\quad
-2e_j\sum_{k\neq j} p_k\,S_{jk}w_k
-e_j\sum_{k\neq j} e_k\,S_{jk}w_k.
\end{align*}

The exact bias formula consists of one term that is quadratic in $p$,
\[
-2p_j\sum_{k\neq j} p_k\,S_{jk}w_k,
\]
and additional terms involving $e$, which arise from replacing $p$ by $\hat p$ in the thinning step. Thus the ideal Richardson correction retains an $O(\|p\|^2)$ bias, while the plug-in step contributes an additional error of order $\|e\|$.

More precisely, for fixed $w\in\RR^d$, the vector
\[
\EE[\hat g^{\mathrm R}_{\hat p}(w)]-\nabla L(w)
\]
is a sum of terms that are quadratic in $p$, linear in $e$, bilinear in $(p,e)$, or quadratic in $e$. Hence, 
\[
\left\|
\EE[\hat g^{\mathrm R}_{\hat p}(w)]-\nabla L(w)
\right\|
\le
c_1(w,S)\|p\|^2
+
c_2(w,S,b)\|e\|
+
c_3(w,S)\|p\|\,\|e\|
+
c_4(w,S)\|e\|^2.
\]
Absorbing the mixed and quadratic terms into the linear term in $\|e\|$, we obtain
\[
\left\|
\EE[\hat g^{\mathrm R}_{\hat p}(w)]-\nabla L(w)
\right\|
=
O\left(\|p\|^2+\|e\|\right) = 
O\left(\|p\|^2+\|\hat p-p\|\right).
\]



\newpage 

\subsection{A MAR extension: scalable observed-score missingness}

The next result shows that the Richardson mechanism extends beyond MCAR, provided the missingness probabilities are driven by an always-observed variable and vary through a scalar intensity parameter.

\begin{theorem}[Richardson under scalable MAR]
\label{thm:richardson-mar}
Let $U$ be an always-observed random variable. For $t\ge 0$, assume that, conditionally on $U$,
\begin{itemize}
    \item $m^{(t)}_1,\dots,m^{(t)}_d$ are mutually independent;
    \item $m^{(t)}$ is independent of $(x,y)$ given $U$;
    \item
    \[
    \PP(\omega_j^{(t)}=0\mid U)=t\,q_j(U),
    \qquad j=1,\dots,d,
    \]
    where $0\le tq_j(U)<1/2$ almost surely. \fg{La encore, généraliser avec $<1$ et Richardson avec couple quelconque pour ne pas se restreindre à $1/2$.}
\end{itemize}
Then, for each coordinate $j$,
\[
\EE[\hat g_j^{(t)}(w)]-\nabla_jL(w)
=
-t\,\EE\big[q_j(U)\,g_j(w;x,y)\big]
-t\,\EE\Big[\sum_{k\neq j} q_k(U)\,x_jx_k w_k\Big]
+t^2\,\EE\Big[q_j(U)\sum_{k\neq j}q_k(U)\,x_jx_k w_k\Big].
\]
Now define an additional thinning mask $r=(r_1,\dots,r_d)$ by
\[
r_j\mid U \sim \mathrm{Bernoulli}\left(\frac{1-2tq_j(U)}{1-tq_j(U)}\right),
\qquad j=1,\dots,d,
\]
independently across coordinates and conditionally independent of $(x,y,m^{(t)})$ given $U$.
Then the Richardson estimator
\[
\hat g^{\mathrm R}(w):=2\hat g^{(t)}(w)-\hat g^{(2t)}(w)
\]
satisfies
\[
\EE[\hat g_j^{\mathrm R}(w)]-\nabla_jL(w)
=
-2t^2\,\EE\Big[q_j(U)\sum_{k\neq j}q_k(U)\,x_jx_k w_k\Big].
\]
In particular, the first-order term is exactly cancelled under this MAR model.
\end{theorem}

\begin{proof}
Condition on $U$. Given $U$, the mask is heterogeneous MCAR with coordinate-wise missingness probabilities
\[
p_j(U)=tq_j(U).
\]
Therefore, by Corollary~\ref{cor:population-bias} applied conditionally on $U$,
\[
\EE[\hat g_j^{(t)}(w)\mid U]-\EE[g_j(w;x,y)\mid U]
=
-p_j(U)\,\EE[g_j(w;x,y)\mid U]
-(1-p_j(U))\sum_{k\neq j}p_k(U)\,\EE[x_jx_k\mid U]\,w_k.
\]
Substituting $p_j(U)=tq_j(U)$ and expanding,
\begin{align*}
\EE[\hat g_j^{(t)}(w)\mid U]-\EE[g_j(w;x,y)\mid U]
&=
-tq_j(U)\,\EE[g_j(w;x,y)\mid U] \\
&\quad
-t\sum_{k\neq j}q_k(U)\,\EE[x_jx_k\mid U]\,w_k \\
&\quad
+t^2 q_j(U)\sum_{k\neq j}q_k(U)\,\EE[x_jx_k\mid U]\,w_k.
\end{align*}
Taking total expectation gives the first formula.

For the second part, note that, conditionally on $U$,
\[
\PP(\omega_j^{(2t)}=1\mid U)
=
\PP(\omega_j^{(t)}=1\mid U)\PP(r_j=1\mid U)
=
(1-tq_j(U))\frac{1-2tq_j(U)}{1-tq_j(U)}
=
1-2tq_j(U).
\]
Thus the further-thinned mask has the same conditional law as the original mask with $t$ replaced by $2t$. Therefore, conditioning on $U$ and using the same expansion with $t$ and $2t$, the linear term cancels:
\[
2m_j(U;t)-m_j(U;2t)
=
-2t^2 q_j(U)\sum_{k\neq j}q_k(U)\,\EE[x_jx_k\mid U]\,w_k,
\]
where $m_j(U;t)$ denotes the conditional bias given $U$. Taking total expectation yields
\[
\EE[\hat g_j^{\mathrm R}(w)]-\nabla_jL(w)
=
-2t^2\,\EE\Big[q_j(U)\sum_{k\neq j}q_k(U)\,x_jx_k w_k\Big].
\]
\end{proof}

The previous theorem shows that MAR is compatible with Richardson extrapolation only when one can scale the \emph{conditional} missingness probabilities. In general, the marginal vector $p=(p_1,\dots,p_d)$ is not sufficient.


\subsection{A self-masked MNAR extension}

A similar argument also works under a structured MNAR model, provided the missingness score is known on observed entries.

\fg{Surement directement mettre l'extension MAR/MNAR agnostique comme c'est la même. }
\fg{Bien sur, on peut de nouveau faire l'estimation de la fonction $q$ et donc retrouver les même taux que quand on estimait le vecteur de proba manquantes en MCAR. }
\begin{theorem}[Richardson under self-masked MNAR]
\label{thm:richardson-mnar}
Let $U$ be an always-observed random variable. For $t\ge 0$, assume that, conditionally on $(x,y,U)$,
\begin{itemize}
    \item $m^{(t)}_1,\dots,m^{(t)}_d$ are mutually independent;
    \item
    \[
    \PP(\omega_j^{(t)}=0\mid x,y,U)=t\,q_j(U,x_j),
    \qquad j=1,\dots,d,
    \]
    where $0\le tq_j(U,x_j)<1/2$ almost surely.
\end{itemize}
Then, for each coordinate $j$,
\[
\EE[\hat g_j^{(t)}(w)]-\nabla_jL(w)
=
-t\,\EE\big[q_j(U,x_j)\,g_j(w;x,y)\big]
-t\,\EE\Big[\sum_{k\neq j} q_k(U,x_k)\,x_jx_k w_k\Big]
+t^2\,\EE\Big[q_j(U,x_j)\sum_{k\neq j}q_k(U,x_k)\,x_jx_k w_k\Big].
\]

Assume moreover that, whenever $\omega_j^{(t)}=1$, one can generate a further thinning variable
\[
r_j\mid (U,x_j,\omega_j^{(t)}=1)\sim
\mathrm{Bernoulli}\left(\frac{1-2tq_j(U,x_j)}{1-tq_j(U,x_j)}\right),
\]
independently across coordinates and conditionally independent given $(x,y,U,m^{(t)})$, and define
\[
\omega_j^{(2t)}:=\omega_j^{(t)}r_j.
\]
Then the Richardson estimator satisfies
\[
\EE[\hat g_j^{\mathrm R}(w)]-\nabla_jL(w)
=
-2t^2\,\EE\Big[q_j(U,x_j)\sum_{k\neq j}q_k(U,x_k)\,x_jx_k w_k\Big].
\]
\end{theorem}

\begin{proof}
Given $(x,y,U)$, the mask coordinates are independent Bernoulli variables with
\[
p_j=tq_j(U,x_j).
\]
Therefore Proposition~\ref{prop:sample-bias}, applied conditionally on $(x,y,U)$, gives
\[
\EE[\hat g_j^{(t)}(w)\mid x,y,U]-g_j(w;x,y)
=
-p_j g_j(w;x,y)
-(1-p_j)\sum_{k\neq j}p_k\,x_jx_k w_k.
\]
Substituting $p_j=tq_j(U,x_j)$ and expanding yields
\begin{align*}
\EE[\hat g_j^{(t)}(w)\mid x,y,U]-g_j(w;x,y)
&=
-tq_j(U,x_j)g_j(w;x,y) \\
&\quad
-t\sum_{k\neq j}q_k(U,x_k)x_jx_k w_k \\
&\quad
+t^2 q_j(U,x_j)\sum_{k\neq j}q_k(U,x_k)x_jx_k w_k.
\end{align*}
Taking expectation over $(x,y,U)$ proves the first identity.

For the further-thinned mask, whenever $\omega_j^{(t)}=1$,
\[
\PP(\omega_j^{(2t)}=1\mid x,y,U)
=
\PP(\omega_j^{(t)}=1\mid x,y,U)\PP(r_j=1\mid x,y,U,\omega_j^{(t)}=1),
\]
hence
\[
\PP(\omega_j^{(2t)}=1\mid x,y,U)
=
(1-tq_j(U,x_j))\frac{1-2tq_j(U,x_j)}{1-tq_j(U,x_j)}
=
1-2tq_j(U,x_j).
\]
So, conditionally on $(x,y,U)$, the second-stage mask is again of the same form with $t$ replaced by $2t$. Applying the previous expansion at levels $t$ and $2t$, and taking
\[
2m_j(x,y,U;t)-m_j(x,y,U;2t),
\]
the linear terms cancel and only
\[
-2t^2 q_j(U,x_j)\sum_{k\neq j}q_k(U,x_k)x_jx_k w_k
\]
remains. Taking total expectation gives the claimed formula.
\end{proof}




\section{MICE Study}
\fg{Surement pas intéressant et à enlever. }

\section{ Linear regression: One missing covariate and one-step linear imputation}


We now specialize the previous analysis to the case where only one feature has missing values. This allows a particularly transparent comparison between zero imputation and one-step linear-regression imputation.

Write the covariate vector as
\[
x=(u,v)\in \RR\times \RR^{d-1},
\]
where $u=x_1$ is the only partially observed feature, and define
\[
m\sim \mathrm{Bernoulli}(1-p),
\qquad m\perp (x,y),
\]
so that $u$ is missing with probability $p\in[0,1)$.

For squared loss,
\[
\ell(w;x,y)=\frac12 (w^\top x-y)^2,
\qquad
g(w;x,y)=(w^\top x-y)x.
\]

We consider a generic \emph{linear imputer}
\[
\hat u = a^\top v,
\qquad a\in\RR^{d-1},
\]
and define the imputed covariate
\[
\tilde x^{(a)} := \bigl(mu+(1-m)a^\top v,\; v\bigr).
\]
The corresponding gradient is
\[
\hat g^{(a)}(w;\tilde x^{(a)},y)
:=
\bigl(w^\top \tilde x^{(a)}-y\bigr)\tilde x^{(a)}.
\]

This framework contains zero imputation as the special case $a=0$.

It is convenient to introduce the imputation residual
\[
e_a := u-a^\top v.
\]
Then
\[
\tilde x^{(a)} = x-(1-m)e_a e_1,
\]
where $e_1=(1,0,\dots,0)^\top\in\RR^d$.

\subsection{Sample-conditional bias under one-step linear imputation}

We first fix one observation $(x,y)$. All expectations in this subsection are taken only over the mask $m$.

\begin{proposition}[Sample-conditional bias]
\label{prop:one-missing-linear-imputation}
Fix $(x,y)\in\RR^d\times\RR$. Then
\[
\EE_m\left[\hat g^{(a)}(w;\tilde x^{(a)},y)\mid x,y\right]-g(w;x,y)
=
-p\,e_a\Bigl(w_1x+(w^\top x-y)e_1\Bigr)
+p\,w_1e_a^2 e_1.
\]
Equivalently, for the first coordinate,
\[
\EE_m\left[\hat g^{(a)}_1(w;\tilde x^{(a)},y)\mid x,y\right]-g_1(w;x,y)
=
-p\,e_a\bigl((w^\top x-y)+w_1a^\top v\bigr),
\]
and for each $j\neq 1$,
\[
\EE_m\left[\hat g^{(a)}_j(w;\tilde x^{(a)},y)\mid x,y\right]-g_j(w;x,y)
=
-p\,w_1 e_a x_j.
\]
\end{proposition}

\begin{proof}
Let
\[
r:=w^\top x-y.
\]
Since $\tilde x^{(a)}=x-(1-m)e_a e_1$,
\[
\hat g^{(a)}(w;\tilde x^{(a)},y)
=
\bigl(r-(1-m)w_1e_a\bigr)\bigl(x-(1-m)e_a e_1\bigr).
\]
Expanding gives
\[
\hat g^{(a)}(w;\tilde x^{(a)},y)-g(w;x,y)
=
-(1-m)e_a\Bigl(w_1x+r e_1\Bigr)
+(1-m)w_1e_a^2 e_1.
\]
Taking expectation over $m$ and using $\EE[1-m]=p$ yields the vector formula.

The coordinatewise expressions follow immediately. For $j\neq 1$, the term involving $e_1$ vanishes, so
\[
\EE_m[\hat g^{(a)}_j\mid x,y]-g_j(w;x,y)=-p\,w_1 e_a x_j.
\]
For $j=1$,
\[
\EE_m[\hat g^{(a)}_1\mid x,y]-g_1(w;x,y)
=
-p\,e_a(w_1u+r)+p\,w_1e_a^2
=
-p\,e_a\bigl(r+w_1(u-e_a)\bigr),
\]
and since $u-e_a=a^\top v$, this becomes
\[
-p\,e_a\bigl((w^\top x-y)+w_1a^\top v\bigr).
\]
\end{proof}

\begin{corollary}[Zero imputation]
\label{cor:zero-imputation-one-missing}
When $a=0$, one recovers zero imputation. Since $e_0=u$, Proposition~\ref{prop:one-missing-linear-imputation} becomes
\[
\EE_m[\hat g^{(0)}_1(w;\tilde x^{(0)},y)\mid x,y]-g_1(w;x,y)
=
-p\,g_1(w;x,y),
\]
and for each $j\neq 1$,
\[
\EE_m[\hat g^{(0)}_j(w;\tilde x^{(0)},y)\mid x,y]-g_j(w;x,y)
=
-p\,w_1u x_j.
\]
\end{corollary}

\subsection{Population bias and comparison with zero imputation}

Let
\[
B^{(a)}(w):=\EE[\hat g^{(a)}(w;\tilde x^{(a)},y)]-\EE[g(w;x,y)].
\]
Also write
\[
S=\EE[xx^\top]
=
\begin{pmatrix}
S_{11} & S_{1,-1}\\
S_{-1,1} & S_{-1,-1}
\end{pmatrix}.
\]

\begin{corollary}[Population bias under one-step linear imputation]
\label{cor:population-bias-one-missing-linear}
For the linear imputer $a$, the population bias satisfies
\[
B^{(a)}_{-1}(w)
=
-p\,w_1\,\EE[e_a v]
=
-p\,w_1\bigl(S_{-1,1}-S_{-1,-1}a\bigr),
\]
and
\[
B^{(a)}_1(w)
=
-p\,\EE\left[e_a\bigl((w^\top x-y)+w_1a^\top v\bigr)\right].
\]
In particular, for zero imputation $a=0$,
\[
B^{(0)}_1(w)=-p\,\nabla_1L(w),
\qquad
B^{(0)}_{-1}(w)=-p\,S_{-1,1}w_1.
\]
\end{corollary}

\begin{proof}
Take expectation with respect to the data distribution in Proposition~\ref{prop:one-missing-linear-imputation}. For $j\neq 1$,
\[
B^{(a)}_j(w)
=
-p\,w_1\,\EE[e_a x_j].
\]
Since $x_j$ is a coordinate of $v$,
\[
\EE[e_a v]
=
\EE[(u-a^\top v)v]
=
S_{-1,1}-S_{-1,-1}a,
\]
which gives the formula for $B^{(a)}_{-1}(w)$. The expression for $B^{(a)}_1(w)$ is obtained directly from the first-coordinate formula in Proposition~\ref{prop:one-missing-linear-imputation}.

When $a=0$, one has $e_0=u$, so
\[
B^{(0)}_{-1}(w)=-p\,w_1\EE[uv]=-p\,S_{-1,1}w_1.
\]
Moreover,
\[
B^{(0)}_1(w)
=
-p\,\EE[u(w^\top x-y)]
=
-p\,\EE[g_1(w;x,y)]
=
-p\,\nabla_1L(w).
\]
\end{proof}

\subsection{Optimal linear imputation}

Among linear imputers, the natural choice is the population least-squares predictor
\[
a_\star := S_{-1,-1}^{-1}S_{-1,1}.
\]
Let
\[
e_\star := u-a_\star^\top v.
\]
By the normal equations,
\[
\EE[e_\star v]=0.
\]

\begin{corollary}[Bias after one optimal linear-regression imputation step]
\label{cor:optimal-linear-imputation}
For $a=a_\star$,
\[
B^{(a_\star)}_{-1}(w)=0,
\qquad
B^{(a_\star)}_1(w)=-p\,\EE\left[e_\star(w^\top x-y)\right].
\]
Hence one optimal linear-regression imputation step removes the bias on all fully observed coordinates; only the coordinate corresponding to the partially observed feature remains biased.
\end{corollary}

\begin{proof}
By definition of $a_\star$,
\[
\EE[e_\star v]=0.
\]
Thus Corollary~\ref{cor:population-bias-one-missing-linear} yields
\[
B^{(a_\star)}_{-1}(w)=0.
\]
Also,
\[
B^{(a_\star)}_1(w)
=
-p\,\EE\left[e_\star\bigl((w^\top x-y)+w_1a_\star^\top v\bigr)\right].
\]
Since $\EE[e_\star a_\star^\top v]=a_\star^\top \EE[e_\star v]=0$, this reduces to
\[
B^{(a_\star)}_1(w)=-p\,\EE\left[e_\star(w^\top x-y)\right].
\]
\end{proof}

\begin{corollary}[Correctly specified linear model]
\label{cor:correct-linear-model-one-missing}
Assume
\[
y=\beta^\top x+\xi,
\qquad
\EE[\xi\mid x]=0.
\]
Then, for the optimal linear imputer $a_\star$,
\[
B^{(a_\star)}_{-1}(w)=0,
\qquad
B^{(a_\star)}_1(w)
=
-p\,(w_1-\beta_1)\,\sigma_{1\mid -1}^2,
\]
where
\[
\sigma_{1\mid -1}^2:=\EE[e_\star^2]
=
S_{11}-S_{1,-1}S_{-1,-1}^{-1}S_{-1,1}.
\]
In particular,
\[
B^{(a_\star)}(\beta)=0.
\]
\end{corollary}

\begin{proof}
By Corollary~\ref{cor:optimal-linear-imputation},
\[
B^{(a_\star)}_1(w)
=
-p\,\EE[e_\star(w^\top x-y)].
\]
Under the model,
\[
w^\top x-y=(w-\beta)^\top x-\xi.
\]
Therefore,
\[
\EE[e_\star(w^\top x-y)]
=
(w-\beta)^\top \EE[e_\star x]-\EE[e_\star\xi].
\]
Since $\EE[e_\star v]=0$ and $\EE[\xi\mid x]=0$,
\[
\EE[e_\star\xi]=\EE\left[e_\star\EE[\xi\mid x]\right]=0.
\]
Moreover,
\[
\EE[e_\star x]
=
\begin{pmatrix}
\EE[e_\star u]\\
\EE[e_\star v]
\end{pmatrix}
=
\begin{pmatrix}
\EE[e_\star^2]\\
0
\end{pmatrix},
\]
because $u=e_\star+a_\star^\top v$. Hence
\[
\EE[e_\star(w^\top x-y)]
=
(w_1-\beta_1)\EE[e_\star^2],
\]
which proves the claim.
\end{proof}

\paragraph{Interpretation.}
With one missing feature, zero imputation creates a bias both on the missing coordinate and on all other coordinates correlated with it. After one optimal linear-regression imputation step, the latter bias disappears. The remaining bias is proportional to the residual variance $\sigma_{1\mid -1}^2$, that is, to the part of the missing feature that cannot be linearly predicted from the fully observed ones.

